Beyond the Known: Decision Making with Counterfactual Reasoning Decision Transformer

Decision Transformers (DT) play a crucial role in modern reinforcement learning, leveraging offline datasets to achieve impressive results across various domains. However, DT requires high-quality, comprehensive data to perform optimally. In real-world applications, the lack of training data and the scarcity of optimal behaviours make training on offline datasets challenging, as suboptimal data can hinder performance. To address this, we propose the Counterfactual Reasoning Decision Transformer (CRDT), a novel framework inspired by counterfactual reasoning. CRDT enhances DT ability to reason beyond known data by generating and utilizing counterfactual experiences, enabling improved decision-making in unseen scenarios. Experiments across Atari and D4RL benchmarks, including scenarios with limited data and altered dynamics, demonstrate that CRDT outperforms conventional DT approaches. Additionally, reasoning counterfactually allows the DT agent to obtain stitching abilities, combining suboptimal trajectories, without architectural modifications. These results highlight the potential of counterfactual reasoning to enhance reinforcement learning agents' performance and generalization capabilities.

==> input/input_exp/modified_env.tex <==

We further evaluate CRDT's generalizability by testing its performance in modified environments, where the dynamics differ from those in the $D_\text{env}$ dataset generated by the behaviour policy $\pi_\beta$. Out of the four environments tested, in Table.~\ref{tab:performance_comparison_modified_env} Appendix~\ref{modified_env}, CRDT improves DT's performance in three. In contrast, REINF shows weaker results in these environments, likely due to its architecture, which forces it to maximize returns within $D_\text{env}$—a condition that may not hold in the modified environments. CRDT excels compared to the original DT method because it generates additional counterfactual experiences, enabling it to cover a broader range of scenarios than the $D_\text{env}$ dataset alone.
    
